Dynamic Membership for Regular Languages

We study the dynamic membership problem for regular languages: fix a language L, read a word w, build in time O(|w|) a data structure indicating if w is in L, and maintain this structure efficiently under letter substitutions on w. We consider this problem on the unit cost RAM model with logarithmic word length, where the problem always has a solution in O(log |w| / log log |w|) per operation. We show that the problem is in O(log log |w|) for languages in an algebraically-defined, decidable class QSG, and that it is in O(1) for another such class QLZG. We show that languages not in QSG admit a reduction from the prefix problem for a cyclic group, so that they require {\Omega}(log |w| / log log |w|) operations in the worst case; and that QSG languages not in QLZG admit a reduction from the prefix problem for the multiplicative monoid U 1 = {0, 1}, which we conjecture cannot be maintained in O(1). This yields a conditional trichotomy. We also investigate intermediate cases between O(1) and O(log log |w|). Our results are shown via the dynamic word problem for monoids and semigroups, for which we also give a classification. We thus solve open problems of the paper of Skovbjerg Frandsen, Miltersen, and Skyum [30] on the dynamic word problem, and additionally cover regular languages.

==> schema.tex <==
\tikzstyle{class}=[inner sep=1em, align=center, ]
\tikzstyle{helper}=[color=white]
\tikzstyle{complexity}=[inner sep=0.2em, scale=1.4]
\tikzstyle{polygone}=[opacity=0.08, line width=3px]
\begin{tikzpicture}[>=stealth]
    \graph[layered layout,  level distance=10em, sibling sep=18em, grow=up, edge quotes mid,
			edges={nodes={fill=white, inner sep=5pt}},
			nodes={color=black, inner sep=1em, draw, text=white, text width=8em, minimum height=4em}]{
		ACom 	-> ["$ab$", bend left=20]				MNil,
		ACom	-> ["$(aa)^*$", bend right=20	]				Com,
		Com 	-> ["$ab$"				]				ZG,
		MNil	-> ["$(aa)^*$", ]				ZG,
		MNil	-> ["$a^*b$"					]				A,
		ZG		-> ["$a^*b$", ]				ZGA,
		ZG		-> ["$(aa)^*b(aa)^*$"			]				ZE,
		ZE		-> ["$(aa)^*ba^*$", bend right		]				All,
		ZGA		-> ["$((abc)^2 )^*((acb)^2)^*$"	]				SG,
		A		-> ["$(aa)^*$"					]				ZGA,
		SG		-> ["$(aa)^*b(aa)^*$", bend left=20]				All,
    };
\node[class] (LACom) at (ACom) {$\ACom$\\$\veq{xy=yx}\land \A$};
\node[class] (LCom) at (Com) {$\Com$\\$\veq{xy=yx}$};
\node[class] (LMNil) at (MNil) {$\MNil$\\$= \ZG\land \A$};
\node[class] (LZG) at (ZG) {$\ZG=\SG\cap\ZE$\\$= \MNil \lor \Com$\\\veq{$x^{\omega+1}y=yx^{\omega+1}}$};
\node[class] (LZE) at (ZE) {$\ZE$\\$\veq{x^{\omega}y=yx^\omega}$};
\node[class] (LZGA) at (ZGA) {$\ZGA$};
\node[class] (LA) at (A) {$\A$\\$\veq{x^{\omega+1}=x^\omega}$};
\node[class,text width=10em] (LSG) at (SG) {$\SG$\\$\veq{x^{\omega+1}yx^\omega=x^\omega y x^{\omega+1}}$};
\node[class, text width=3cm, fill=none] (LAll) at (All) {\bfseries All monoids};
\node[helper] (X) at (Com.south east) [xshift=1em] {X};
\node[helper] (Y) at (X.center |- ZG.north) [yshift=0.5em] {Y};
\node[helper] (Z) at (X.center |- ZE.north)[yshift=2em] {Z};
\node[helper] (LX) at (MNil.south west) [xshift=-1em] {LX};
\node[helper] (LY) at (LX |- MNil.north)[yshift=0.5em] {LY};
\node[helper] (LZ) at (LX |- SG.north)[yshift=0.5em] {LZ};




\draw[draw=green!50!black, fill=green, polygone ] (X.center) -- (Y.center) -- (ZG.north west |- Y) -- (MNil.north east|-LY.center) -- (LY.center) -- (LX.center) -- (ACom.south west) -- (ACom.south east) -- cycle;
\node[complexity] (cst) at (ACom.north) [anchor=south, yshift=1.7em,] {$\mathcal{O}(1)$};

\draw[draw=blue!50!black, fill=blue, polygone] (Y.center) -- (SG.north east |- LZ.center) --  (LZ.center) -- (LY.center) -- (MNil.north east |- LY.center) --(ZG.north west |- Y)-- cycle;
\node[complexity] (cst2) at (LZGA.east) [anchor=west, xshift=2.5em, text width=10em, align=center] {$\mathcal{O}(\log\log n)$\\prefix-$U_1$ hard};

\draw[draw=red!50!black, fill=red, polygone] (LZ.center) -- (All.north west) --  (All.north east) -- (Z.center) -- (Y.center) -- (SG.north east |- LZ.center) --cycle;
\node[complexity] (cst3) at (All.south) [anchor=north, yshift=-2em, text width=10em, align =center]
	{$\Theta(\log n/\log\log n)$\\ prefix-$\ZZ_d$ hard};
\end{tikzpicture}

